Ab-Initio Solution of the Many-Electron Schr\"odinger Equation with Deep Neural Networks

Given access to accurate solutions of the many-electron Schr\"odinger equation, nearly all chemistry could be derived from first principles. Exact wavefunctions of interesting chemical systems are out of reach because they are NP-hard to compute in general, but approximations can be found using polynomially-scaling algorithms. The key challenge for many of these algorithms is the choice of wavefunction approximation, or Ansatz, which must trade off between efficiency and accuracy. Neural networks have shown impressive power as accurate practical function approximators and promise as a compact wavefunction Ansatz for spin systems, but problems in electronic structure require wavefunctions that obey Fermi-Dirac statistics. Here we introduce a novel deep learning architecture, the Fermionic Neural Network, as a powerful wavefunction Ansatz for many-electron systems. The Fermionic Neural Network is able to achieve accuracy beyond other variational quantum Monte Carlo Ans\"atze on a variety of atoms and small molecules. Using no data other than atomic positions and charges, we predict the dissociation curves of the nitrogen molecule and hydrogen chain, two challenging strongly-correlated systems, to significantly higher accuracy than the coupled cluster method, widely considered the most accurate scalable method for quantum chemistry at equilibrium geometry. This demonstrates that deep neural networks can improve the accuracy of variational quantum Monte Carlo to the point where it outperforms other ab-initio quantum chemistry methods, opening the possibility of accurate direct optimization of wavefunctions for previously intractable many-electron systems.

==> references.tex <==

%% Put the bibliography here, most people will use BiBTeX in
%% which case the environment below should be replaced with
%% the \bibliography{} command.

\begin{thebibliography}{1}
\bibitem{troyer2005complexity} Troyer, M. \& Wiese, U.J. Computational complexity and fundamental limitations to fermionic quantum Monte Carlo simulations. {\em Phys. Rev. Lett.}, {\bf 94}(17), 170201 (2005).

\bibitem{krizhevsky2012imagenet} Krizhevsky, A., Sutskever, I. \& Hinton, G. E. Imagenet classification with deep convolutional neural networks. {\em NeurIPS}, 1097–1105 (2012).

%\bibitem{silver2016mastering} Silver, D., Huang, A., Maddison, C. J., Guez, A., Sifre, L., Van Den Driessche, G., Schrittwieser, J., Antonoglou, I., Panneershelvam, V., Lanctot, M., Dieleman, S., Grewe, D., Nham, J., Kalchbrenner, N., Sutskever, I., Lillicrap, T., Leach, M., Kavukcuoglu, K., Graepel, T. \& Hassabis, D. Mastering the Game of Go with Deep Neural Networks and Tree Search. {\em Nature}, {\bf 529}(7587), 484 (2016).

\bibitem{silver2016mastering} Silver, D., et al. Mastering the game of Go with deep neural networks and tree search. {\em Nature}, {\bf 529}, 484-489 (2016).

\bibitem{carleo2017solving} Carleo, G. \& Troyer, M. Solving the quantum many-body problem with artificial neural networks. {\em Science}, {\bf 355}, 602-606 (2017).

\bibitem{bartlett2007coupled} Bartlett, R. J. \& Musiał, M. Coupled-cluster theory in quantum chemistry. {\em Rev. Modern Phys.}, {\bf 79}, 291 (2007).

\bibitem{gilmer2017neural} Gilmer, J., Schoenholz, S. S., Riley, P. F., Vinyals, O. \& Dahl, G.E. Neural message passing for quantum chemistry. {\em ICML}, 1263-1272 (2017).

\bibitem{schutt2019unifying} Sch\"utt, K. T., Gastegger, M., Tkatchenko, A., M\"uller, K.-R. \& Maurer, R. J. Unifying machine learning and quantum chemistry with a deep neural network for molecular wavefunctions. {\em Nat. Commun.}, {\bf 10}, 5024 (2019).

\bibitem{mills2017deep} Mills, K., Spanner, M. \& Tamblyn, I. Deep learning and the Schr{\"o}dinger equation. {\em Phys. Rev. A}, {\bf 96}(4), 042113 (2019).

\bibitem{sinitskiy2019physical} Sinitskiy, A. V. \& Pande, V. S. Physical machine learning outperforms ``human learning" in quantum chemistry. {\em arXiv preprint arXiv:1908.00971} (2019).

\bibitem{cheng2019universal} Cheng, L., Welborn, M., Christensen, A. S., \& Miller III, T. F., A universal density matrix functional from molecular orbital-based machine learning: Transferability across organic molecules. {\em J. Chem. Phys.}, {\bf 150}, 113103 (2019).

\bibitem{born1927zur} Born, M. \& Oppenheimer, R. Zur Quantentheorie der Molekeln. {\em Annalen der Physik}, {\bf 389}, 457-484 (1927).

\bibitem{booth2010approaching} Booth, G. H. \& Alavi, A. Approaching chemical accuracy using full configuration-interaction quantum Monte Carlo: a study of ionization potentials. {\em J. Chem. Phys.}, {\bf 132}, 174104 (2010).

\bibitem{foulkes2001quantum} Foulkes, W. M. C., Mitas, L., Needs, R. J. \& Rajagopal, G. Quantum Monte Carlo simulations of solids. {\em Rev. Modern Phys.}, {\bf 73}, 33 (2001).

\bibitem{feynman1956energy} Feynman, R.P. \& Cohen, M. Energy spectrum of the excitations in liquid helium. {\em Phys. Rev.}, {\bf 102}(5), 1189 (1956).

\bibitem{bajdich2006pfaffian} Bajdich, M., Mitas, L., Drobný, G., Wagner, L.K. \& Schmidt, K.E. Pfaffian pairing wave functions in electronic-structure quantum Monte Carlo simulations. {\em Phys. Rev. Lett.}, {\bf 96}, 130201 (2006).

\bibitem{orus2014practical} Or\'{u}s, R., A practical introduction to tensor networks: Matrix product states and projected entangled pair states. {\em Ann. Phys.}, {\bf 349}, 117 (2014). 

\bibitem{choo2018symmetries} Choo, K., Carleo, G., Regnault, N. \& Neupert, T. Symmetries and many-body excitations with neural-network quantum states. {\em Phys. Rev. Lett.}, {\bf 121}, 167204 (2018).

\bibitem{nagy2019variational} Nagy, A. \& Savona, V. Variational quantum Monte Carlo method with a neural-network Ansatz for open quantum systems. {\em Phys. Rev. Lett.}, {\bf 122}, 250501 (2019).

\bibitem{nomura2017restricted} Nomura, Y., Darmawan, A. S., Yamaji, Y. \& Imada, M. Restricted Boltzmann machine learning for solving strongly correlated quantum systems. {\em Phys. Rev. B}, {\bf 96}, 205152 (2017).

\bibitem{yang2019deep} Yang, L., et al. Deep learning-enhanced variational Monte Carlo method for quantum many-body physics. {\em arXiv preprint arXiv:1905.10730}

\bibitem{luo2019backflow} Luo, D. \& Clark, B. K. Backflow transformations via neural networks for quantum many-body wave functions. {\em Phys. Rev. Lett.}, {\bf 122}, 226401 (2019).

\bibitem{saito2018method} Saito, H. Method to solve quantum few-body problems with artificial neural networks. {\em J. Phys. Soc. Japan}, {\bf 87}(7), 074002 (2018).

\bibitem{kessler2019artificial} Kessler, J., Calcavecchia, C. \& K{\"u}hne, T. D. Artificial neural networks as trial wave functions for quantum Monte Carlo. {\em arXiv preprint arXiv:1904.10251} (2019).

\bibitem{han2018solving} Han, J., Zhang, L. \& E, W. Solving many-electron Schr{\"o}dinger equation using deep neural networks. {\em arXiv preprint arXiv:1807.07014} (2018).

\bibitem{taddei2015iterative} Taddei, M., Ruggeri, M., Moroni, S. \& Holzmann, M. Iterative backflow renormalization procedure for many-body ground state wave functions of strongly interacting normal Fermi liquids. {\em Phys. Rev. B}, {\bf 91}, 205152 (2015).

\bibitem{ruggeri2018nonlinear} Ruggeri, M., Moroni, S. \& Holzmann, M. Nonlinear Network description for many-body quantum systems in continuous space. {\em Phys. Rev. Lett.}, {\bf 120}, 205302 (2018).

\bibitem{hermann2019deep} Hermann, J., Sch{\"a}tzle, Z. \& No{\'e}, F. Deep neural network solution of the electronic Schr{\"o}dinger equation. {\em arXiv preprint arXiv:1909.08423} (2019).

\bibitem{choo2019fermionic} Choo, K., Mezzacapo, A. \& Carleo, G. Fermionic neural-network states for ab-initio electronic structure. {\em arXiv preprint arXiv:1909.12852} (2019).

\bibitem{zhang2018abinitio} Zhang, S. Ab Initio Electronic Structure Calculations by Auxiliary-Field Quantum Monte Carlo. In {\em Handbook of Materials Modeling} (Springer, Cham, 2018).

\bibitem{shawetaylor1989building} Shawe-Taylor, J. Building symmetries into feedforward networks. {\em ICANN}, 158-162 (1989).

\bibitem{martens2015optimizing} Martens, J., \& Grosse, R. Optimizing neural networks with Kronecker-factored approximate curvature. {\em ICML}, 2408-2417 (2015).

\bibitem{sorella1998green} Sorella, S. Green function Monte Carlo with stochastic reconfiguration. {\em Phys. Rev. Lett.}, {\bf 80}, 4558 (1998).

\bibitem{otis2019complementary} Otis, L. and Neuscamman, E. Complementary first and second derivative methods for Ansatz optimization in variational Monte Carlo. {\em Phys. Chem. Chem. Phys.}, {\bf 21}, 14491-14510 (2019).

\bibitem{seth2011quantum} Seth, P., Ríos, P. L. \& Needs, R. J. Quantum Monte Carlo study of the first-row atoms and ions. {\em J. Chem. Phys.}, {\bf 134}, 084105 (2011).

\bibitem{chakravorty1993ground} Chakravorty, S. J., Gwaltney, S. R., Davidson, E. R., Parpia, F. A. \& Fischer, C. F. Ground-state correlation energies for atomic ions with 3 to 18 electrons. {\em Phys. Rev. A}, {\bf 47}, 3649 (1993).

\bibitem{klopper2010submev} Klopper, W., Bachorz R. A., Tew D. P., and Hättig C. Sub-meV accuracy in first-principles computations of the ionization potentials and electron affinities of the atoms H to Ne. {\em Phys. Rev. A} {\bf 81}, 022503 (2010).

\bibitem{giner2016qmc} Giner, E. \& Assaraf, R. \& Toulouse, J.Quantum Monte Carlo with reoptimised perturbatively selected configuration-interaction wave functions. {\em Mol. Phys.}, {\bf 114}, 910-920 (2016).

\bibitem{dash2018perturbatively} Dash, M., Moroni, S., Scemama, A. \& Filippi, C. Perturbatively selected configuration-interaction wave functions for efficient geometry optimization in quantum Monte Carlo. {\em J. Chem. Theory Comput.}, {\bf 14}, 4176-4182 (2018).

\bibitem{filippi1996multiconfiguration} Filippi, C. \& Umrigar, C.J. Multiconfiguration wave functions for quantum Monte Carlo calculations of first‐row diatomic molecules. {\em J. Chem. Phys.}, {\bf 105}, 213-226 (1996).

\bibitem{cencek2000benchmark} Cencek, W. \& Rychlewski, J. Benchmark calculations for He2+ and LiH molecules using explicitly correlated gaussian functions. {\em Chem. Phys. Lett.}, {\bf 320}, 549-552 (2000).

\bibitem{vanvoorhis2000benchmark} Van Voorhis, T. \& Head-Gordon, M. Benchmark variational coupled cluster doubles results. {\em J. Chem. Phys.}, {\bf 113}, 8873-8879 (2000).

\bibitem{burton2016holomorphic} Burton, H. G. A., Thom, A. J. W. Holomorphic Hartree–Fock Theory: An Inherently Multireference Approach. {\em J. Chem. Theory Comput.} {\bf 12} 167 (2016).

\bibitem{lyakh2011multireference} Lyakh, D. I., Musiał, M., Lotrich, V. F. \& Bartlett, R. J. Multireference nature of chemistry: the coupled-cluster view. {\em Chem. Rev.}, {\bf 112}, 182-243 (2011).

\bibitem{leroy2006accurate} Le Roy, R. J., Huang, Y. \& Jary, C. An accurate analytic potential function for ground-state N$_2$ from a direct-potential-fit analysis of spectroscopic data. {\em J. Chem. Phys.}, {\bf 125}, 164310 (2006).

\bibitem{gdanitz1998accurately} Gdanitz, R. J. Accurately solving the electronic Schrödinger equation of atoms and molecules using explicitly correlated ($r_{12}$-)MR-CI: the ground state potential energy curve of N2. {\em Chem. Phys. Lett.}, {\bf 283}, 253-261 (1998).

%\bibitem{darwent1970bond} Darwent, B. D. Bond dissociation energies in simple molecules. {\em National Standard Reference Data System}, NSRDS-NBS-31 (1970).

%\bibitem{irikura2007experimental} Irikura, K. K. Experimental vibrational zero-point energies: Diatomic molecules. {\em J. Phys. Chem. Ref. Data}, {\bf 36}(2), 389-397 (2007).

%\bibitem{motta2017towards} Motta, M., Ceperley, D. M., Chan, G. K. L., Gomez, J. A., Gull, E., Guo, S., Jiménez-Hoyos, C. A., Lan, T. N., Li, J., Ma, F., Millis, A. J., Prokof'ev, N. V., Ray, U., Scuseria, G. E., Sorella, S., Stoudenmire, E. M., Sun, Q., Tupitsyn, I. S., White, S. R., Zgid, D. \& Zhang, S. Towards the Solution of the Many-Electron Problem in Real Materials: Equation of State of the Hydrogen Chain with State-of-the-Art Many-Body Methods. {\em Physical Review X}, {\bf 7}(3), 031059 (2017).

\bibitem{motta2017towards} Motta, M., et al. Towards the solution of the many-electron problem in real materials: equation of state of the hydrogen chain with state-of-the-art many-body methods. {\em Phys. Rev. X}, {\bf 7}, 031059 (2017).

\end{thebibliography}
